Lyman-alpha radiation pressure: an analytical exploration

We study radiation pressure due to Lyman alpha line photons, obtaining and exploring analytical expressions for the force-multiplier, $M_F(N_H, Z) = F_\alpha/(L_\alpha/c)$, as a function of gas column density, $N_H$, and metallicity, $Z$, for both dust-free and dusty media, employing a WKB approach for the latter case. Solutions for frequency offset emission to emulate non-static media moving with a bulk velocity $v$, have also been obtained. We find that, in static media, Ly$\alpha$ pressure dominates over both photoionization and dust-mediated UV radiation pressure in a very wide parameter range ($16 < \log N_H < 23$; $-4 < \log[Z/Z_\odot] < 0$). For example, it overwhelms the other two forces by 10 (300) times in standard (low-$Z$) star-forming clouds. Thus, in agreement with previous studies, we conclude that Ly$\alpha$ pressure plays a dominant role in the initial acceleration of the gas around luminous sources, and must be implemented in galaxy formation, evolution and outflow models and simulations.

==> Lya Radiation Pressure/definitions.tex <==

%%%%% AUTHORS - PLACE YOUR OWN COMMANDS HERE %%%%%

% Please keep new commands to a minimum, and use \newcommand not \def to avoid
% overwriting existing commands. Example:
%\newcommand{\pcm}{\,cm$^{-2}$}	% per cm-squared

% definitions by GMT
%\usepackage[T1]{fontenc}
%\usepackage[utf8]{inputenc}
%\usepackage[italian,english]{babel}
%\usepackage{amsmath,amssymb,mathtools,braket}
%\newcommand{\ped}[1]{\textormath{\textsubscript{#1}}{_{\mathrm{#1}}}}
%\newcommand{\ap}[1]{\textormath{\textsuperscript{#1}}{^{\mathrm{#1}}}}
%\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
%\renewcommand{\vec}{\mathbf}
%\newcommand{\dd}{\mathop{\mathrm{d}\!}{}}
%\DeclareMathOperator\artanh{artanh}
%\DeclareMathOperator\Li{Li}

% quick alias
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\newcommand\code[1]{\textsc{\MakeLowercase{#1}}}
\newcommand\quotesingle[1]{`{#1}'}
\newcommand\quotes[1]{``{#1}"}
\def\gsim{\lower.5ex\hbox{\gtsima}} 
\def\lsim{\lower.5ex\hbox{\ltsima}} 
\def\gtsima{$\; \buildrel > \over \sim \;$} 
\def\ltsima{$\; \buildrel < \over \sim \;$} \def\gsim{\lower.5ex\hbox{\gtsima}} 
\def\lsim{\lower.5ex\hbox{\ltsima}} 
\def\simgt{\lower.5ex\hbox{\gtsima}} 
\def\simlt{\lower.5ex\hbox{\ltsima}} 


% solar stuff units
\def\msun{{\rm M}_{\odot}}
\def\lsun{{\rm L}_{\odot}}
\def\dsun{{\cal D}_{\odot}}
\def\fsun{\xi_{\odot}}
\def\zsun{{\rm Z}_{\odot}}
\def\msunyr{\msun/{\rm yr}}
% units
\def\mum{\mu {\rm m}}
\newcommand{\angstrom}{\mbox{\normalfont\AA}}
\def\cc{\rm cm^{-3}}
\def\uflux{{\rm erg}\,{\rm s}^{-1} {\rm cm}^{-2} }
% quantities defs
\def\fdust{\xi_{d}}
\def\fesc{f_{\rm esc}}
\def\td{\tau_{sd}}
% additional wrappers for quantities and untis
\def\Dsolar{${\cal D}/\dsun$}
\def\Zsolar{$Z/\zsun$}
\def\DDsolar{\left( {{\cal D}\over \dsun} \right)}
\def\ZZsolar{\left( {Z \over \zsun} \right)}

% LINES
\def\S*{$\Sigma_{\rm SFR}$}
\def\Scii{$\Sigma_{\rm [CII]}$}
\def\Sciimax{$\Sigma_{\rm [CII]}^{\rm max}$}
\def\CII{\hbox{[C~$\scriptstyle\rm II $]~}}
\def\CIII{\hbox{C~$\scriptstyle\rm III $]~}}
\def\Lya{Ly$\alpha$}
%\def\CII{[CII]~} 
%\def\CIII{CIII]~}
% IONS
\def\HH{\hbox{H$_2$}~} 
\def\HI{\hbox{H~$\scriptstyle\rm I\ $}} 
\def\HII{\hbox{H~$\scriptstyle\rm II\ $}} 
\def\CIion{\hbox{C~$\scriptstyle\rm I $~}}
\def\CIIion{\hbox{C~$\scriptstyle\rm II $~}}
\def\CIIIion{\hbox{C~$\scriptstyle\rm III $~}}
\def\CIVion{\hbox{C~$\scriptstyle\rm IV $~}}
% ion variables
\def\nhh{n_{\rm H2}}
\def\nhi{n_{\rm HI}}
\def\nhii{n_{\rm HII}}
\def\fhh{x_{\rm H2}}
\def\fhi{x_{\rm HI}}
\def\fhii{x_{\rm HII}}
% MIX
\def\fd{f^*_{\rm diss}} 
\def\ks{\kappa_{\rm s}}

% COLORS
\def\cyan{\color{cyan}}
\definecolor{apcolor}{HTML}{b3003b}
\definecolor{afcolor}{HTML}{800080}
\definecolor{lvcolor}{HTML}{DF7401}
\definecolor{mdcolor}{HTML}{01abdf} %mahsa and davide
\definecolor{cbcolor}{HTML}{ff0000}
\definecolor{sccolor}{HTML}{cc5500} %stefano
\definecolor{sgcolor}{HTML}{00cc7a}

% ADDED BY G.M.TOMASELLI:
% 1) Correctly typeset the "d" of differentials:
\newcommand{\dd}{\mathop{\mathrm{d}\!}{}}
% 2) Shorthands for roman text in sup/sub-scripts:
\newcommand{\ped}[1]{_{\mathrm{#1}}}
\newcommand{\ap}[1]{^{\mathrm{#1}}}
% 3) Rendering for vectors and versors:
\renewcommand{\vec}[1]{\boldsymbol{\mathbf{#1}}}
\newcommand{\ver}[1]{\vec{\hat #1}}
% 4) artanh:
\DeclareMathOperator{\artanh}{artanh}
\DeclareMathOperator{\Li}{Li}
% 5) absolute value:
%\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}

==> Lya Radiation Pressure/pack.tex <==

% MNRAS is set in Times font. If you don't have this installed (most LaTeX
% installations will be fine) or prefer the old Computer Modern fonts, comment
% out the following line
\usepackage{newtxtext,newtxmath}
% Depending on your LaTeX fonts installation, you might get better results with one of these:
%\usepackage{mathptmx}
%\usepackage{txfonts}

% Use vector fonts, so it zooms properly in on-screen viewing software
% Don't change these lines unless you know what you are doing
\usepackage[T1]{fontenc}
\usepackage{ae,aecompl}

%%%%% AUTHORS - PLACE YOUR OWN PACKAGES HERE %%%%%

% Only include extra packages if you really need them. Common packages are:
\usepackage{graphicx}	% Including figure files
\usepackage{amsmath}	% Advanced maths commands
%\usepackage{amssymb}	% Extra maths symbols
\usepackage[nameinlink,noabbrev]{cleveref}

\usepackage{xcolor}

\usepackage[separate-uncertainty=true,multi-part-units=single]{siunitx}
